Signature-Based Abduction for Expressive Description Logics -- Technical Report

Signature-based abduction aims at building hypotheses over a specified set of names, the signature, that explain an observation relative to some background knowledge. This type of abduction is useful for tasks such as diagnosis, where the vocabulary used for observed symptoms differs from the vocabulary expected to explain those symptoms. We present the first complete method solving signature-based abduction for observations expressed in the expressive description logic ALC, which can include TBox and ABox axioms, thereby solving the knowledge base abduction problem. The method is guaranteed to compute a finite and complete set of hypotheses, and is evaluated on a set of realistic knowledge bases.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
As discussed in \cite{elsenboich2006case}, KB abduction generalises both the TBox abduction and ABox abduction problems, rather than considering the two to be entirely separate. Our approach instead tackles the general KB problem directly, rather than simply addressing the TBox and ABox abduction problems as two separate cases simultaneously, as illustrated by Example \ref{ex:kb-example}:
\begin{example}\label{ex:kb-example}
Let $\Kmc=\{A \sqsubseteq \forall r.B, \lnot C(b)\}$, $\Psi = \forall r.C(a)$ and $\Sig = \{A, B, C\}$. The solution returned by the approach in this paper is $\hyp = \{B \sqsubseteq C, A(a)\}$
\end{example}

Thus, the proposed approach will produce a more general hypothesis containing a TBox for a purely ABox observation if it is required as part of an optimal solution, i.e., it is done cautiously particularly with respect to the semantic minimality condition.

